Lossy Lorentz boosts at ultra-relativistic energies: Numerical study and source survey of high-energy physics software

Most high-energy-physics software packages implement Lorentz boosts for themselves. At sufficiently large boosts, these routines can return finite, plausible-looking four-vectors whose invariant masses and rest-frame properties are no longer accurate. We survey implementations in widely used collider and air-shower software and compare representative algorithms in three numerical tests. We find that the main problem is usually information discarded by the representation, rather than the arithmetic of the boost formula. Information can be lost when a boost is specified only by its velocity, and again when the result is stored only through Cartesian components. Richer boost input prevents the first loss, while retaining light-cone coordinates prevents the second. Ordinary hard processes at present colliders are safe in double precision; the relevant regimes are low-mass systems, highly boosted auxiliary frames, single-precision particle records and air-shower simulations. Extreme scale hierarchies in parton-shower accuracy tests and ultra-heavy particle decays provide still more demanding cases.

==> figs/timing.tex <==
A1 & 4.4 \\
A2 & 5.8 \\
A3 & 1.7 \\
A4, one shot & 2.4 \\
A4, retained & 0.6 \\

